"With Great Power Comes Great Responsibility!": Student and Instructor Perspectives on the influence of LLMs on Undergraduate Engineering Education

The rise in popularity of Large Language Models (LLMs) has prompted discussions in academic circles, with students exploring LLM-based tools for coursework inquiries and instructors exploring them for teaching and research. Even though a lot of work is underway to create LLM-based tools tailored for students and instructors, there is a lack of comprehensive user studies that capture the perspectives of students and instructors regarding LLMs. This paper addresses this gap by conducting surveys and interviews within undergraduate engineering universities in India. Using 1306 survey responses among students, 112 student interviews, and 27 instructor interviews around the academic usage of ChatGPT (a popular LLM), this paper offers insights into the current usage patterns, perceived benefits, threats, and challenges, as well as recommendations for enhancing the adoption of LLMs among students and instructors. These insights are further utilized to discuss the practical implications of LLMs in undergraduate engineering education and beyond.

==> files/04b-old-faculty-evaluation.tex <==
\subsubsection{\textbf{Initial Exposure to ChatGPT}}\hfill\\
% instructors were introduced to ChatGPT through various channels such as word-of-mouth, media coverage, and discussions with peers. 
Participants initially learned about ChatGPT through conversations with peers, friends, and colleagues as well as through news articles and reports. Some participants were interviewed by news channels or publications, further increasing their exposure to ChatGPT. The general online presence and enthusiasm around ChatGPT also caught the attention of the participants and made them try out ChatGPT on their own.
% Faculty groups within universities discussed about ChatGPT, where members shared insights, experiences, and discussed its potential impact on education.
% \begin{quote}
% All of a sudden everyone was talking about ChatGPT. We have this faculty group within the university where multiple faculty members started sending emails about ChatGPT and how it is a big revaluation revolution in AI and it is able to answer any type of question! When some discussion starts in the faculty group, then everyone chimes in and people started talking about how ChatGPT is able to solve all the programming assignments, how ChatGPT solved a question which we thought it could not. This made me interested in wanting to explore ChatGPT! -[T15]
% \end{quote}
% Many participants came across articles and news reports that highlighted ChatGPT's capabilities.

% \begin{quote}
% Nine to ten months ago, at that time, I think I was in Switzerland when I had a telephonic interview with a German news channel. I don't know how they got my phone number, but they called me while I was in Switzerland, and I gave an interview that was out there in public. So, that's the time when I read more about it. -[T8]
% \end{quote}
% \begin{quote}
% I came across ChatGPT because of the hype it generated on the internet. It was crazy, so like everyone else, I also tried my hand at it. -[T9]
% \end{quote}
% \subsubsection{\textbf{What was the intial reaction of instructors?}}
% Participants expressed a range of reactions and experiences upon learning about ChatGPT.

Some participants initially viewed it as a potentially overhyped technology and questioned its practical utility. One participant even compared ChatGPT to the early days of Google, suggesting that its initial results might not be perfect as was the case with Google. On the other hand, several participants were impressed and enthusiastic about ChatGPT's capabilities, especially in terms of information retrieval, summarization and problem-solving. There were also some participants who praised ChatGPT for its ability to summarize information effectively and provide answers to some questions but at the same time, also noted inaccuracies and limitations in handling certain types of queries such as solving numerical problems. Some participants expressed worries that ChatGPT might encourage students to rely on it for ready-made answers rather than genuinely learning and understanding the subject matter.
% \begin{quote}
% I fell in love with it. Wow, I mean, it was simply amazing. Nobody would have thought things like that were possible. -[T3]
% \end{quote}


% \begin{quote}
% ChatGPT's theoretical explanations are fine, as they summarize things nicely. However, sometimes, they also miss out on valuable information. In such cases, it's not a good idea to rely on this chatbot for solving numerical problems. Numerical problems can be challenging, and if you try to twist them, it will be difficult to solve them using this chatbot. - [T6]
% \end{quote}

% \begin{quote}
% I figured out that ChatGPT could not even solve the most basic questions involving math and symbols. It did try to provide some answers, but apart from one of the very, very basic ones, which you could easily find on the internet, it could only give real answers. The other answers it provided were not in proper English and didn't make mathematical sense. -[T10]
% \end{quote}

% Some participants also raised concerns about the potential impact of ChatGPT on education and learning. 
\subsubsection{\textbf{Awareness about Student Usage of ChatGPT}}\hfill\\
Many participants admitted that they are not fully aware of how students are using ChatGPT in their courses. Some of them did express an intention to initiate discussions with students to gain a better understanding of their experience with ChatGPT. Some participants also mentioned that the nature of the take-home assignments in their courses is such that they did not think ChatGPT would be able to solve them. Hence, they did not feel the need of any discussion with students. On the other hand, some participants were aware of students trying to use ChatGPT in open-internet exams and assignments. Some participants were also concerned that students are blindly using ChatGPT's responses without even understanding whether they are meaningful or not. Some of them even caught such students red-handed.
\begin{quote}
Even in the labs, we observed students blindly copying code for tasks related to communication systems, which may be fine.But the problem is that they don't really understand what they're copying. They just want to get the work done. It undermines the learning of the students. -[T16] 
\end{quote} 

% \begin{quote}
% My assignments are more on the creative side, where students need to curate their own data or engage in more creative tasks. So, I've never actually had a lengthy discussion with anyone on ChatGPT. -[T3]
% \end{quote}

% \begin{quote}
% I teach subjects that involve numerical problems, and I know that they cannot be solved through ChatGPT. Therefore, I'm not very concerned about discussing those topics with the students. -[T6]
% \end{quote}



% \begin{quote}
% When I teach programmable networking, students were attempting to use the open internet during my exams to find answers and write code. However, they were completely unsuccessful, and their answers turned out to be incorrect. What I heard from the students is that they never benefited from it because they were unable to find the answers. I think this is specifically due to the nature of the course. However, if it were a more common course like networks, which I am teaching right now, I believe they should be able to find answers more easily.-[T14]
% \end{quote}



\subsubsection{\textbf{Constructive Use of ChatGPT by Students}}\hfill\\
\textbf{Enhancing Learning Through ChatGPT.} Participants shared that \textbf{ChatGPT can complement students already proficient in a subject}, aiding them in learning more about that subject. However, its reliability may not suffice for critical assignments, necessitating students to have a background in the topic to identify inaccuracies. Some participants also believed that \textbf{ChatGPT can help in focused and efficient learning} by providing concise, specific information, and directing students to relevant resources about any topic. This saves them valuable time that might otherwise be spent searching through numerous sources. Participants also thought that \textbf{ChatGPT can simplify complex concepts}, making them accessible to students with varying levels of subject proficiency and helping bridge language barriers. Some participants also mentioned that the \textbf{ChatGPT platform offers a distraction-free and safe learning environment}, devoid of advertisements and providing controlled access to reliable information, particularly beneficial for young learners. Finally, some participants also believed that the \textbf{interactive and user-friendly interface of ChatGPT enables iterative learning and reinforcement}. Students can receive assistance, identify mistakes, and improve their understanding through back-and-forth interactions. Additionally, \textbf{ChatGPT supports experimentation and exploration of "what if" scenarios} on a particular topic for deeper comprehension. Participants also mentioned that students can leverage \textbf{ChatGPT to generate practice questions on any topic}. This can enable students to create their own exercises based on course material, promoting a deeper understanding of concepts. In this context, a participant highlighted that ChatGPT may sometimes provide incorrect answers to a question. \textbf{This discrepancy can be used as an opportunity to debate with peers on the correctness of the answer}, ultimately, contributing to enhanced learning and a deeper comprehension of course material.
\begin{quote}
    If students use it efficiently, it can really help them learn things in a very focused manner. In classroom teaching, we have limited time, so we can't delve into every topic in great detail. At the same time, we don't expect students to go through every topic in depth. Some topics are crucial, some we want them to skim through, and some we want them to explore with a bit more depth. The advantage of ChatGPT is that it doesn't overload you with a lot of information; it provides very focused information on a specific topic. This can be very satisfying for a student, and they can feel confident that they've understood that topic. The level of detail is also not overwhelming for a student, so in that way, it can help students learn in a focused manner. Instead of searching on Google, where they might get 15 or 20 results and have to decide which one is the most appropriate for focused learning, ChatGPT provides a more streamlined experience. - [T4]
\end{quote}
% \begin{quote}
%     Before the mid-semester exam, after covering the theory, students can utilize ChatGPT to generate practice questions, attempt to solve them on their own, and then seek solutions from ChatGPT. If their answer doesn't match ChatGPT's answer, it can lead to an interesting aspect. ChatGPT is just an AI model, so students can't be certain whether ChatGPT's answer is correct or not. This discrepancy can provide an excellent opportunity for discussion with fellow classmates. For example, ChatGPT is giving answer X, but my answer is Y. Let's discuss whether X or Y is correct. This can lead to further learning and productive discussions among students. - [T15]
% \end{quote}

\noindent\textbf{Using ChatGPT as a writing and coding assistant.} Participants saw ChatGPT as a valuable tool for \textbf{enhancing students' academic and professional writing skills, particularly pertinent for those whose first language is not English (such as students in India)}. It offers grammar, structure, and presentation suggestions for research papers, articles, emails, and other written communication. Additionally, ChatGPT can provide guidance on the process of writing research papers and even generate templates. A participant expressed that \textbf{exposure to high-quality written material generated by ChatGPT can also contribute to improved spoken communication}. Participants also believed that ChatGPT serves as a resource for students struggling with expressing mathematical ideas clearly. It can generate well-structured outlines for proving theorems, \textbf{aiding students in developing the skill of writing mathematical proofs effectively}. Many participants mentioned that ChatGPT can assist students in generating basic code for assignments or projects, \textbf{serving as a starting point to save time and effort}. However, some participants had concerns about over-reliance on ChatGPT. They recommended that ChatGPT should be used for coding assistance only from sophomore year or later so that students can grasp fundamental programming concepts.
\begin{quote}
    In my courses, we often have to prove theorems and establish various facts, some of which may not always be very extensive but still require careful articulation. When I provide ChatGPT with an outline of the proof, it can generate a well-structured and elegantly written proof. For instance, when dealing with standard proof techniques like induction or contradiction, the way ChatGPT formulates the proofs is often superior to what an average second-year undergraduate student could produce. This skill of effectively communicating solutions or proofs is something that everyone should have. Even if you know the answer or solution, being able to convey it clearly and elegantly is essential. From my limited interaction, I believe that students should make the most of this capability...[...]..I am confident that with the right structure and guidance, ChatGPT can assist them in this aspect. - [T13]
\end{quote}

\noindent\textbf{Using ChatGPT Responsibly.} Participants emphasize that students should understand that \textbf{ChatGPT is a tool to aid their learning, not a replacement for their intellectual capabilities}. It's important for students to use ChatGPT responsibly and not rely on it excessively. For example, ChatGPT could be used for small or trivial parts of assignments or when students need quick assistance, but not as a complete substitute for their own learning efforts.

\begin{quote}
    If students understand that an assignment is meant for them to grasp the concepts, and they use ChatGPT for the right purpose, like for a small, trivial part or to save time on certain aspects, I think that's fine. But if they rely on ChatGPT for the entire assignment, then I believe it's a problem. - [T12]
\end{quote}  

% \textbf{Complementary Tool for Those with Prior Knowledge.} Some participants believed that ChatGPT can be valuable for students who already possess some knowledge of a subject. For example, students with programming skills, can use ChatGPT to quickly validate code or save time by generating code snippets. ChatGPT may not be suitable for students attempting to complete assignments or understand complex subjects they have not studied before. Participants mentioned that ChatGPT's responses may contain errors or lack reliability, making it unsuitable for critical assignments. It's important for students to have a background in the topic they are querying to identify inaccuracies or mistakes made by ChatGPT.

% \begin{quote}
%     Like when you do a Google search, you get a lot of options, and there are many reliable links, such as Wikipedia, that you can rely on. With ChatGPT, you don't know how it's obtaining that information; there's no source. So, from that perspective, I'm a bit skeptical. However, if you already possess some knowledge and then use ChatGPT, it could be helpful. For instance, if you're already well-versed in programming and can identify whether something is a correct program or not, then using ChatGPT to save time and effort makes sense. I think from that perspective, ChatGPT is useful. -[T12]
% \end{quote}

% \begin{quote}
%     It's not like a student who has never studied operating systems can use ChatGPT to solve an operating system assignment; it's not going to work that way. If a student attempts that, they will easily be caught because ChatGPT more often than not makes mistakes, and these mistakes are quite obvious. There's a difference between human mistakes and AI mistakes, so it's easy to figure out whether a mistake was made by a human or AI. - [T15]
% \end{quote}

% \noindent\textbf{Focused and Efficient Learning.} Participants mentioned that ChatGPT can help students learn topics in a more focused manner. In traditional classroom settings, there's often limited time to cover every detail. In such scenarios, ChatGPT  can help students to gain a deeper understanding of the topics covered in the classroom by providing concise and specific information, without being overwhelmed. Additionally, ChatGPT enables efficient learning. It provides answers quickly and directs students to the most relevant resources, saving them valuable time that might otherwise be spent searching through numerous sources. This is especially useful when they need quick answers or summaries. One participant mentioned that ChatGPT can also be useful for students who wish to engage in research but lack the background knowledge. Faculty members can provide such students with specific research topics and then these students can use ChatGPT to look up reading materials, explanations, and guidance on these research topics. Another participant proposed using ChatGPT to address the issue of prerequisites for courses. Rather than having a strict prerequisite requirement for a course, ChatGPT could provide students with the necessary foundational materials and quizzes to ensure they have the required knowledge. This could make education more accessible and flexible. 

% \begin{quote}
%     If students use it efficiently, it can really help them learn things in a very focused manner. In classroom teaching, we have limited time, so we can't delve into every topic in great detail. At the same time, we don't expect students to go through every topic in depth. Some topics are crucial, some we want them to skim through, and some we want them to explore with a bit more depth. The advantage of ChatGPT is that it doesn't overload you with a lot of information; it provides very focused information on a specific topic. This can be very satisfying for a student, and they can feel confident that they've understood that topic. The level of detail is also not overwhelming for a student, so in that way, it can help students learn in a focused manner. Instead of searching on Google, where they might get 15 or 20 results and have to decide which one is the most appropriate for focused learning, ChatGPT provides a more streamlined experience. - [T4]
% \end{quote}

% \noindent\textbf{Simplifying Complex Concepts.} Participants mentioned that ChatGPT can simplify complex concepts, making them more accessible to students with varying levels of proficiency in a subject. It can help bridge language barriers and ensure that all students can grasp the material.

% \begin{quote}
%     Sometimes it also simplifies things because if you ask it to explain in a simpler way, it simplifies the concept, making it accessible to students who may not be very proficient in the language. So, in that sense, it's beneficial. However, students have the responsibility to ensure that they understand the concept. - [T16]
% \end{quote}

% \noindent\textbf{Distraction-Free and Safe Learning.} Participants mentioned that ChatGPT can provide a safer and more controlled learning environment for students. This includes the absence of distracting advertisements commonly found on many websites. Absence of advertisements enhance concentration and reduce exposure to potentially inappropriate or misleading content. Additionally, ChatGPT can help protect users, particularly young learners, from fake news and unreliable sources on the internet by delivering information in a controlled manner, thereby promoting the consumption of accurate and trustworthy content. In other words, it can alleviate some of the risks associated with unrestricted internet browsing.

% \begin{quote}
%     You know, with ChatGPT, you're not exposed to a lot of ads, and you're saved from all those internet ills like fake pages and fake news, right? So, at least from a benefit perspective, I feel that it's good in that aspect. - [T19]
% \end{quote}

% \noindent\textbf{Interactive and User-Friendly Interface.} Some participants also believe that ChatGPT's interactive interface can be more user-friendly than traditional search engines, providing information in a conversational manner.

% \begin{quote}
%     You can use ChatGPT because the interface is a bit easier, right? It communicates in a more interactive way. On the other hand, Google's interface isn't as user-friendly; you get a bunch of links and have to figure out where to find the information you're looking for. So, yeah, from that perspective, I think ChatGPT is still useful. - [T12]
% \end{quote}

% \noindent\textbf{Iterative Learning and Reinforcement Learning using ChatGPT.} The interactive interface of ChatGPT can also enable iterative and reinforcement learning. For instance, students preparing for coding interviews can use ChatGPT interactively. They may start by attempting to solve coding problems independently. If they encounter difficulties or get stuck while solving a problem, they can turn to ChatGPT for assistance. ChatGPT can provide assistance to students by identifying mistakes in their code. Students then review the identified mistakes and attempt to fix them on their own. They may repeat this process several times to improve their code. This back-and-forth interaction allows for iterative learning and problem-solving. Furthermore, a participant mentioned that students can use ChatGPT as a tool for reinforcement learning. ChatGPT can be used to experiment with different scenarios and "what if" questions. They can make changes and adjustments to a particular problem statement or system and see how these modifications impact the outcomes. This can give them a deeper understanding of the subject matter.

% \begin{quote}
%     In their senior year when students are preparing for job placements, they can actually use ChatGPT in an interactive manner. For instance, if they are preparing for coding interviews, they can start by attempting a problem and inform ChatGPT that they are working on that particular problem. After writing the code, if they get stuck or encounter errors, they can provide the code to ChatGPT and ask for guidance on identifying the mistakes. ChatGPT can help identify the mistakes but doesn't provide the complete solution. The student then goes back to review the code, tries to fix the issues, and may or may not succeed. They can repeat this process multiple times and then return to ChatGPT to discuss further. This kind of interactive discussion with ChatGPT can be another interesting use case, especially when preparing for final exams and interviews. -[T15]
% \end{quote}

% \noindent\textbf{Improving academic and professional writing skills.} Participants see ChatGPT as a supportive tool that can help students improve their academic and professional writing skills, especially when it comes to research papers and formal communication. This is especially going to be beneficial for students whose first language is not English (such as those in India), ChatGPT can help improve their written English skills by providing suggestions for grammar, structure, and presentation in research papers, articles, emails, or other written communication. For example, ChatGPT can provide step-by-step guidance on how to write research papers. This can be particularly beneficial for undergraduate students who generally don’t have much experience and understanding of the process of writing academic papers. ChatGPT can also assist students by generating templates for research papers, which can serve as a starting point for their own work. One participant mentioned that ChatGPT will ultimately also assist in improving spoken communication as students will be exposed to high quality written material generated by ChatGPT.

% \begin{quote}
%     In the process of writing a research paper, many students and even faculty members often encounter a significant barrier when starting. For such cases, ChatGPT can provide a template to help students begin their writing. They can then proceed to write some of the text themselves. Additionally, ChatGPT can be used to refine the text. For instance, if a student writes a paragraph, especially in countries like India where English is not the native language, ChatGPT can assist in improving grammar, adding more structure to the writing, and fixing presentation errors. Some may view this as an unethical way to use ChatGPT, as it might seem like students are presenting themselves as better English writers than they actually are. However, I believe it's a fair use case because not everyone can be expected to have the same level of proficiency in English as native speakers. Ultimately, when submitting research papers or articles, we are also judged on the quality of our English. - [T15]
% \end{quote}

% \noindent\textbf{Assistance with Mathematical Proof Writing.} Many students struggle with expressing their mathematical ideas clearly, even when they understand the concepts. ChatGPT can serve as a valuable resource to help students overcome this challenge. ChatGPT's ability to generate well-structured outlines for proving theorems can help students develop the essential skill of writing mathematical proofs or explanations in a clear and articulate manner.

% \begin{quote}
%     In my courses, we often have to prove theorems and establish various facts, some of which may not always be very extensive but still require careful articulation. When I provide ChatGPT with an outline of the proof, it can generate a well-structured and elegantly written proof. For instance, when dealing with standard proof techniques like induction or contradiction, the way ChatGPT formulates the proofs is often superior to what an average second-year undergraduate student could produce. This skill of effectively communicating solutions or proofs is something that everyone should have. Even if you know the answer or solution, being able to convey it clearly and elegantly is essential. From my limited interaction, I believe that students should make the most of this capability...[...]..I am confident that with the right structure and guidance, ChatGPT can assist them in this aspect. - [T13]
% \end{quote}

% \noindent\textbf{Generating Boiler Plate Code using ChatGPT.} Participants also suggested that students can use ChatGPT to generate basic code for an assignment or project to have  a starting point. This can save time and effort. ChatGPT can assist in generating code snippets, algorithms, or templates. At the same time, participants had concerns that it might hinder the understanding of fundamental concepts. They mentioned that if freshmen students rely too heavily on ChatGPT, they might miss out on the opportunity to explore and understand the basics of programming. Hence, they recommended that students begin using ChatGPT for coding assistance, perhaps in their sophomore year or later.

% \begin{quote}
%     They can have some basic code generated, and then they can build upon it. This approach can be beneficial, especially for projects where achieving the desired results quickly is important. ChatGPT can help with some of the basic aspects, reducing the need to start programming from scratch. However, for students in their first-year courses, if they start relying on ChatGPT too early, they might miss out on the opportunity to explore why certain things like 'import stdio.h' are necessary. In that sense, it may not serve its purpose of augmenting the power of human learning if it's used by those who should be focusing on fundamental concepts. Students could use ChatGPT as a starting point, but I would recommend doing so only after their first year, maybe in the second year of their studies. - [T9]
% \end{quote}

% \noindent \textbf{Using ChatGPT for generating practice questions.} Participants also discussed how students can benefit from using ChatGPT in the context of closed-book proctored exams. To perform well in such exams, students must understand the concepts and practice problems based on the studied concepts. Participants mentioned that ChatGPT can be utilized by students as a tool to generate practice questions. In addition to the practice questions provided by the instructor, students can use ChatGPT to create practice questions related to the course material. Once generated, students can attempt to solve these practice questions independently. If they encounter difficulties or have doubts, they can turn to ChatGPT for solutions. However, the participant raised an interesting point that ChatGPT may not always provide correct answers, and this discrepancy can lead to valuable discussions among students. When ChatGPT's answers don't align with the student's solutions, it provides an opportunity for students to engage in discussions with their peers. They can debate on the correctness of answers, which can lead to enhanced learning and deeper understanding of the course material.

% \begin{quote}
%     Before the mid-semester exam, after covering the theory, students can utilize ChatGPT to generate practice questions, attempt to solve them on their own, and then seek solutions from ChatGPT. If their answer doesn't match ChatGPT's answer, it can lead to an interesting aspect. ChatGPT is just an AI model, so students can't be certain whether ChatGPT's answer is correct or not. This discrepancy can provide an excellent opportunity for discussion with fellow classmates. For example, ChatGPT is giving answer X, but my answer is Y. Let's discuss whether X or Y is correct. This can lead to further learning and productive discussions among students. - [T15]
% \end{quote}

% \noindent\textbf{Encouraging Responsible Use.} Participants emphasize that students should understand that ChatGPT is a tool to aid their learning, not a replacement for their intellectual capabilities. It's important for students to use ChatGPT responsibly and not rely on it excessively. For example, ChatGPT could be used for small or trivial parts of assignments or when students need quick assistance, but not as a complete substitute for their own learning efforts.

% \begin{quote}
%     If students understand that an assignment is meant for them to grasp the concepts, and they use ChatGPT for the right purpose, like for a small, trivial part or to save time on certain aspects, I think that's fine. But if they rely on ChatGPT for the entire assignment, then I believe it's a problem. - [T12]
% \end{quote}  

\subsubsection{\textbf{Threats ChatGPT Poses to Students}}\hfill\\
\textbf{Decreasing Cognitive Skills.} Participants expressed concerns that ChatGPT could tempt students to seek quick answers without investing the time to truly understand the material. This behavior may undermine the learning process as well as academic integrity. A participant mentioned that \textbf{students may view copying from ChatGPT as a less immoral alternative to copying from peers}. Some participants were worried about the \textbf{possible decline in students' intellectual abilities due to over-reliance on ChatGPT}, drawing parallels with technology dependency seen with smartphones and calculators. They feared that \textbf{ChatGPT may discourage systematic learning, critical thinking, problem-solving, and creativity}. Some participants were also concerned that students might become passive consumers of information, diminishing their analytical skills.

\begin{quote}
    There will always be a threat. I don't know if there was a survey conducted by Harvard a few years ago, where they concluded that with the advent of smartphones, human intelligence quotient is decreasing. I can relate to it personally. When I had a basic phone, I could remember six to seven phone numbers in my mind, ready to dial at any time. But now, I can't even remember my wife's phone number. So, what has happened? We've become so dependent on technology that we've stopped using that part of our brain. I suspect that if this dependence on technology goes unchecked, it may lead to a situation where human intelligence is compromised. Students tend to seek the path of least resistance. It might reach a point where students say, "Why should I study now? I can do it later with ChatGPT." This attitude could continue and eventually lead to students trying to use it for unfair advantages in tests or exams. So, any technology should be used in moderation and enjoyed responsibly. -[T3]
\end{quote}

\noindent\textbf{Decreasing social interactions.}  Participants expressed concern that the availability of tools like ChatGPT may reduce students' inclination to seek help from their peers or teachers when they encounter challenges or questions as they may now resort to ChatGPT. This may make the students less social with other students and instructors. Hence, it's important to strike a balance between utilizing technology for assistance and maintaining social interaction and collaborative learning.

\begin{quote}
    It's gradually reducing in that aspect. In the past, when students didn't know something, they would ask their peers or teachers for the solution or the underlying concept. But these interactions seem to be missing these days, and it's kind of unsocializing the students. -[T6]
\end{quote}

\noindent\textbf{Bringing homogeneity in student thinking.} One participant highlighted that if everyone relies on the same AI tool such as ChatGPT for generating content or answers, it could lead to homogeneity in thinking and content production. 
% In other words, students or individuals might end up with similar responses or ideas because they are all using the same AI model.

\begin{quote}
    It might pose a threat of bringing about homogeneity in people's thinking because if everyone relies on ChatGPT or a similar tool for answers, they may end up with similar responses. This could lead to a more homogeneous and less diverse range of perspectives and ideas. It's not just a threat but a broader issue. - [T13]
\end{quote}

% \noindent\textbf{Shortcut to Answers may not be Shortcut to Learning.} Many participants were concerned that the students may be tempted to use ChatGPT as a shortcut to obtain answers to assignments or questions without investing the time to understand the material. This could undermine the learning process and academic integrity. At the same time, one participant also mentioned that students were already copying from each other to some extent. Copying from a machine like ChatGPT appears to be just easier. There might be fewer moral questions associated with using AI-generated content compared to copying from peers. Additionally, one participant argued that it is not clear how relying on ChatGPT or similar tools for answers might impact students' overall learning. While it's acknowledged that not doing the work and simply copying answers from ChatGPT can hinder learning, but it’s long-term impact on students' professional development is uncertain.

% \begin{quote}
%     So, we already believe that all these students copy from each other, right? That's the basic assumption. In that context, this is similar; instead of copying from a fellow student, it's copying from ChatGPT. ChatGPT is like a person, right? Copying from ChatGPT. So, to that extent, it is... Now, the only thing is that for some reason, copying from a machine is morally not as challenging. There are no moral questions involved. The only moral question arises if the faculty member had said, 'Look, don't use it,' and you still use it as a student. But cheating has... Even in that case. So, here, it will be easier. Easier. The student is less likely to have doubts about using it compared to copying from... There are dynamics involved. Will a friend provide it or not, and how will the friend feel that you got marks without working? But when it comes to this, the herd mentality would be similar now. - [T11]
% \end{quote}

% \noindent\textbf{ChatGPT may lead to decline in Intellectual, Creative, Analytical and Thinking Abilities.} Some participants were concerned that over-reliance on ChatGPT may lead to a decline in students' intellectual abilities. They drew a parallel with the use of smartphones and calculators, where people have become dependent on technology for information and memory. They suggested that ChatGPT could have a similar effect on students' learning. Some participants were also afraid that students might become less inclined to engage in systematic learning and critical thinking. Instead of studying topics step by step, students might resort to using ChatGPT to quickly obtain answers, potentially missing out on the deeper understanding of subjects. Participants were also worried that ChatGPT’s usage could hinder students' thinking abilities. The process of solving problems and thinking critically is seen as essential for brain development, and excessive reliance on AI could diminish this skill. There was also a concern that excessive use of ChatGPT may stifle creativity and critical thinking. Instead of generating their own ideas and solutions, students might become passive consumers of information. Participants feared that ChatGPT may also curtail students' analytical skills, as they might rely on the tool to perform analysis and provide results without engaging in the analytical process themselves.

% \begin{quote}
%     There will always be a threat. I don't know if there was a survey conducted by Harvard a few years ago, where they concluded that with the advent of smartphones, human intelligence quotient is decreasing. I can relate to it personally. When I had a basic phone, I could remember six to seven phone numbers in my mind, ready to dial at any time. But now, I can't even remember my wife's phone number. So, what has happened? We've become so dependent on technology that we've stopped using that part of our brain. I suspect that if this dependence on technology goes unchecked, it may lead to a situation where human intelligence is compromised. Students tend to seek the path of least resistance. It might reach a point where students say, "Why should I study now? I can do it later with ChatGPT." This attitude could continue and eventually lead to students trying to use it for unfair advantages in tests or exams. So, any technology should be used in moderation and enjoyed responsibly. - [T3]

%     I think it's going to impact creative and critical thinking. People used to engage their own brains to find solutions and information, which led to different perspectives and solutions. However, now, with tools like ChatGPT, you just write down a question, and you immediately get an answer. We can see this in our own behavior when ChatGPT didn't exist, and we relied on Google. We became a bit reliant on quick answers, which may have impacted our depth of knowledge. Our elders often had vast knowledge stored in their minds, but we started saying, "Let's Google it," and now it might become, "Let's ChatGPT it." I believe this is a warning for the younger generation that they might lose some of their creativity and critical thinking skills. Having too much information readily available might not allow for deep thinking and could potentially reduce creativity. - [T18]
% \end{quote}

% \subsubsection{\textbf{How are instructors utilizing ChatGPT?}}

\subsubsection{\textbf{Augmenting Teaching using ChatGPT}}\hfill\\
\noindent\textbf{Enriching lectures and assessments.} Participants mentioned that instructors can use ChatGPT to enhance their teaching by \textbf{finding alternative explanations for challenging concepts} and \textbf{generating additional examples and practice questions}. This approach can not only aid in conveying information more effectively but can also provide students with practical applications of the material. ChatGPT's generative ability assists in \textbf{creating diverse, up-to-date lecture materials and well-structured assessments}, increasing student engagement and understanding. Participants also explained that ChatGPT can help the instructors generate relevant content within seconds, thus, \textbf{optimizing their teaching efficiency}. Few participants mentioned that \textbf{ChatGPT can also assist in course design by suggesting the most effective sequence of topics} and relevant course material to improve learning outcomes and engagement for students. This saves time in researching and designing course content and also ensures that the course remains up-to-date and relevant. Participants also stressed on the importance of instructors embracing technology and being open to innovation. Rather than resisting technological advancements, \textbf{instructors should leverage tools like ChatGPT to enhance the learning experience for students}. Some participants also encouraged instructors to familiarize themselves with the limitations of online resources like ChatGPT and how these instructor can add value to overcome these limitations. 
\begin{quote}
    A couple of months ago, I was designing a new course related to the performance modeling of communication networks here in the electrical engineering department. We planned to offer this course to our students. While I was preparing for it, my senior colleagues suggested that I should explore other universities' portals to see if they are offering similar courses for their students. This took up a significant amount of my time, and often, I found that the information I came across was not very relevant. When searching for such information, ChatGPT, being more optimized, could save a lot of time in designing course content. For example, once I've finalized a course topic and its content, there might be elements that I'm missing, which could add value and are already taught in similar courses at other universities. If ChatGPT can highlight such relevant information, it would enhance the quality and content of our teaching while also saving time, at least in the process of finding the right resources for the topic. [T16]
\end{quote}

\noindent\textbf{Interactive simulations and assessments.} A computer science instructor suggested that instructors can utilize ChatGPT to create simulators for teaching a system or algorithm. They provided an example of implementing a networking router using ChatGPT and designing prompts in such a way that ChatGPT is able to generate routing entries to be stored in the routing table. This simulation can allow students to explore and assess the router's functionality, particularly in routing packets to the correct interfaces. By using ChatGPT to create such interactive simulations and assessments, instructors can enhance their teaching methods by providing students with practical, hands-on experiences that help them better understand complex systems and algorithms.

\begin{quote}
Implementing a router using ChatGPT was an interesting experiment. The questions were designed in a way that routing entries were being created, and the system had to determine how to route a given packet type to the correct interface. There were instances where it successfully worked, and there were also cases where it was not successful. -[T14]   
\end{quote}

\noindent\textbf{Keeping academic integrity and authenticity intact by "NOT" using ChatGPT.} One participant was of the opinion that using ChatGPT to prepare teaching material is cheating and should be avoided completely. They believed that the teaching material should reflect their genuine understanding and interpretation of the subject matter. They believed in the value of building content from the ground up and citing sources transparently, emphasizing the role of their own scholarship in the teaching process.

\begin{quote}
    Every line I write should reflect something I genuinely believe in, something that has become a part of my understanding. I'm not even copying from textbooks. If I'm not allowed to copy from textbooks, how can I justify copying from ChatGPT? I must think about what the textbooks are conveying, interpret the material, and create my own slides. It should be a product of my scholarship. If I use ChatGPT, it would essentially be cheating. Furthermore, there's the concern of the reliability of sources. As a teacher, I should start from scratch, begin with a textbook, and build my content from the ground up, citing all my sources in my slides. - [T2]
\end{quote}
% \begin{quote}
%     In some of the courses we teach, conventional textbooks may not have the most up-to-date information or examples. For instance, when teaching Systems Engineering, it would be great to provide students with examples like the Chandrayaan 3 mission and explain the launch process using an engineering approach. However, this kind of information might not be covered in traditional textbooks. ChatGPT can help by providing more detailed and current explanations. When we use current examples, the classroom becomes more engaging for students. Repeating traditional examples may not capture the interest of the current generation. There are various reasons why students don't attend classes, but one of them could be that the teaching methods are too conventional. To address this, we have to adapt to the needs of the generation we're teaching. In this regard, ChatGPT can be a helpful tool. - [T4]
% \end{quote}

% \noindent\textbf{Enriching lectures and assessments using ChatGPT to increase student engagement and learning.} Participants mentioned that instructors can interact with ChatGPT to find alternative ways of explaining challenging concepts that are both intuitive and rigorous. This can help instructors convey information more effectively to their students. Further, instructors often use examples and sample questions to illustrate concepts during teaching. Many times, the examples and questions in textbook or other available material are not sufficient. Sometimes, the instructors may want to cover some real-world examples related to the topic so that the students understand the practical applications of the topic as well. In such scenarios, ChatGPT can generate additional examples and questions that cover various cases and scenarios related to a particular topic. These generated examples and questions can be valuable teaching aids to provide students with a deeper understanding of the subject matter. Additionally, many times, the course textbook may not have up-to-date content. In such cases also, ChatGPT can aid instructors in preparing lecture materials by providing up-to-date content. This can also help in increasing the student engagement. The generative ability of ChatGPT could also be utilized in creating diverse and well-structured assessments for their students.

% \begin{quote}
%     I find it really helpful. ChatGPT saves a lot of time when it comes to preparing our slides. It provides us with focused content. Sometimes, students ask questions that we ourselves may not have immediate answers to because becoming experts in a particular field isn't achievable by studying just one book. In such cases, ChatGPT comes to our aid. Additionally, in some of the courses we teach, conventional textbooks may not have the most up-to-date information or examples. For instance, when teaching Systems Engineering, it would be great to provide students with examples like the Chandrayaan 3 mission and explain the launch process using an engineering approach. However, this kind of information might not be covered in traditional textbooks. ChatGPT can help by providing more detailed and current explanations. When we use current examples, the classroom becomes more engaging for students. Repeating traditional examples may not capture the interest of the current generation. There are various reasons why students don't attend classes, but one of them could be that the teaching methods are too conventional. To address this, we have to adapt to the needs of the generation we're teaching. In this regard, ChatGPT can be a helpful tool. - [T4]
% \end{quote}

% \noindent\textbf{Increasing Instructor Efficiency.} Some participants were of the opinion that ChatGPT could be utilized by instructors to quickly gather any kind of information required for teaching a topic. ChatGPT can provide reliable information in a matter of seconds, streamlining the process of preparing engaging lectures or presentations.

% \begin{quote}
%      On the first day of the course, I wanted to provide an anecdote and a historical perspective of the subject. It seemed impossible, and I would have had to spend five days researching to gather all the relevant information about the field's history and how it evolved to its current state. However, ChatGPT provided me with this information in just two seconds, and it turned out to be quite reliable. I even cross-checked it. So, it significantly helps in terms of saving time. - [T8]
% \end{quote}

% \noindent\textbf{Course Design and Planning.} Participants mentioned that ChatGPT can also assist in course design by suggesting the most effective sequence of topics to improve learning outcomes and engagement for students. Further, Instructors can use ChatGPT to find relevant course materials and resources from other universities or institutions that offer similar courses. This saves time in researching and designing course content and ensures that the course remains up-to-date and relevant.

% \begin{quote}
%     "A couple of months ago, I was designing a new course related to the performance modeling of communication networks here in the electrical engineering department. We planned to offer this course to our students. While I was preparing for it, my senior colleagues suggested that I should explore other universities' portals to see if they are offering similar courses for their students. This took up a significant amount of my time, and often, I found that the information I came across was not very relevant. When searching for such information, ChatGPT, being more optimized, could save a lot of time in designing course content. For example, once I've finalized a course topic and its content, there might be elements that I'm missing, which could add value and are already taught in similar courses at other universities. If ChatGPT can highlight such relevant information, it would enhance the quality and content of our teaching while also saving time, at least in the process of finding the right resources for the topic." [T16]
% \end{quote}

% \noindent\textbf{Adopting innovative teaching methods to stay relevant.} Participants emphasized the importance of instructors staying innovative and open to learning, especially when there are so many online resources and technology-driven learning tools such as ChatGPT. Instructors should familiarize themselves with the limitations of online resources, including ChatGPT, to understand where these tools may fall short in providing comprehensive education and how can they add value to overcome the gaps. Rather than resisting technological advancements, instructors should embrace technology as a tool to enhance their teaching methods. They should explore how to leverage tools like ChatGPT to improve the learning experience for their students.

% \begin{quote}
%     These days, everything is available online and when you're teaching, especially in a setting where there's no attendance system, you need to be highly innovative in your teaching approach. If you present the material in a conventional manner, students might not attend your class because they can easily access the same information from YouTube, NPTEL videos, or ChatGPT. To engage students and make your teaching more effective, you have to be innovative. This innovation comes from understanding the limitations of these online sources and figuring out what extra effort you can put in to simplify and explain concepts and theories effectively. Exploring these sources briefly can help you improve in this regard." -[T6]
% \end{quote}

\subsubsection{\textbf{Potential Impact of ChatGPT on Undergraduate Curriculum and Student Assessments}}\hfill\\
\noindent\textbf{Moving Towards Higher-Order Learning.} Some participants expressed the need to adapt learning outcomes and possibly revise course content if ChatGPT's usage becomes pervasive. They mentioned that instructors could move towards higher-order learning and problem-solving while asking students to use ChatGPT for more routine and maintainable tasks. For instance, in a software engineering course, instructors could focus more on advanced concepts and delegate routine tasks, like writing code modules, to ChatGPT. This would allow students to engage with higher-level thinking and problem-solving. However, the participants also acknowledged the challenges of developing such a higher level of understanding without going through the foundational learning processes. For instance, what to remove from existing content/curriculum to accommodate new higher-level concepts. Additionally, adapting learning outcomes and revising course content is based on the assumption that all students will rely on ChatGPT and related tools for the routine or tasks. This may not be the case always.

\begin{quote}
There are no easy answers to that. I lack clarity on this issue. It appears that we need to move towards a higher order of learning, focusing on complex problems and solutions, while using ChatGPT for lower-level, more routine tasks. However, it's still not clear to me how we can achieve a higher level of complexity without going through the foundational learning process. Can we skip this process entirely? My intuition tells me that we cannot develop a deep understanding without going through the process of grasping the fundamentals. It's like trying to become a proficient coder who assembles modules created by ChatGPT without having a solid understanding of the underlying concepts. I'm not entirely sure about the feasibility of that approach. - [T11]    
\end{quote}

\noindent\textbf{Rethinking Student Assessment Strategies in the Age of ChatGPT.} Many participants acknowledged the need to reconsider traditional assessment methods in light of ChatGPT's presence. Participants recognized that in-class closed-book exams are likely to retain their significance in undergraduate assessment due to the controlled and supervised testing environment. This controlled environment helps maintain the integrity of assessments, making them less susceptible to the influence of AI tools like ChatGPT. However, they also acknowledged the importance of supplementary assessment components, such as take-home assignments and projects, to foster deeper engagement with course material. But many participants found open-book or open-internet assessments problematic due to the potential for students to rely on ChatGPT. Some instructors have already eliminated open-book assessments from their courses in response to this challenge. For those who would like to continue having open-book assessments, some participants emphasized the importance of contextualizing questions to prevent ChatGPT from providing ready-made answers. Assignments that require real observations, personal experiences, and synthesis of information could be designed to promote deeper understanding and discourage reliance on AI. Instructors may also adjust the complexity of problems to make them less amenable to ChatGPT-generated solutions.
\begin{quote}
    Earlier, I used to assign term papers, but now I've shifted the focus. I've added more weightage to assignments that require observation and practical involvement. Students need to write about their observations and even take real photos as part of their assignments. They can't simply rely on internet sources for everything. I emphasize these points in my assignments; for example, I ask them to include self-taken photos. This way, I can tell if they've genuinely engaged with the subject matter. I removed the term paper requirement because I know they can easily write it using ChatGPT. Secondly, in design courses, projects and assignments, most of them are not very binary; they involve observation and presentation, such as creating a video. I try to make them as non-objective as possible, so AI may not be as useful in that context. This doesn't mean I make the assignments overly challenging, but analyzing existing products or designs around them can provide valuable insights. -[T19]
\end{quote}

\noindent\textbf{Plagiarism Detection Just Became More Difficult.} 
Participants also believed that open-book assessments are also going to make the task of detecting plagiarism difficult. Instructors will find it challenging to distinguish between original student work and work that may have been generated or heavily influenced by ChatGPT. This raises concerns about the ability to verify students' actual learning when grading such assessments. Further, it is also known that students may modify AI-generated answers to make them appear original. Participants suggested that there is a need for discussion and brainstorming among instructors to address these challenges. They need to explore ways to detect AI tool usage and potentially adapt their evaluation methods to ensure fairness and integrity.

\begin{quote}
    It's difficult as an instructor to figure out answers from ChatGPT, right? I mean, somebody is writing an answer, and I have a moral and academic responsibility of evaluating their answer and giving them credit if it is original and not giving credit if it is not original. But that is very difficult. I mean, in a non-regulated setting, I don't know if you got it, it's not a very hard task to modify a Chat answer to make it look like it's an original. I think it's an important point as an instructor. So I feel that now when I give homework marks to someone, that 10 out of 10 may not actually mean that the student knows the stuff. I'm not able to verify the learning of the student. There is some brainstorming required or discussion required on how to either change the way we detect cheating or change our style of evaluation. -[T10]
\end{quote}

% \noindent\textbf{Rethinking Student Assessment.} Participants believed that ChatGPT will necessitate rethinking how students are assessed. Participants mentioned that in-class closed-book assessments can still be used to assess students but students don't always like such assessments. On the other hand, open-book or open-internet assessments may not be useful as students may directly use ChatGPT to get answers.

% They suggested that assignments should focus on higher intellectual complexities and thought-provoking tasks rather than repetitive or easily answerable questions. This is necessary to remain relevant in an era where students can easily access AI assistance. To counter the use of ChatGPT in assignments, they propose creating assignments that cannot be easily answered using AI tools. This could involve designing more complex and unique problems that require students to engage actively with course material.

% \begin{quote}
% "Why are you making me memorize?" So we are like, "That's true. We don't want to make you memorize." What's the next option? Open book kind of thing or do takeaway assignments. Instead of searching on the Internet, they can get it from ChatGPT. We're trying to increase the takeaway assignments. And now, these tools are not helping us to do that. Moreover, if I ask them in class, it's not just a matter of can I use the Internet or not? How can I justify to them not to use the Internet when they are going to use the Internet in their jobs? How can I say no, you can answer this question without the Internet? Previously, before Chat GPT, I would say, use the Internet. You still won't get the answer without thinking. I'm quite confident of the questions. I can't say that option is taken away from me. I can't be free and say, no, you can't use the Internet. I have to restrict them: don't use anything. Just see my slides or think. How do I justify this to them? And that's an open book component. Open book means what it should be. Open means to the Internet as well. Now I'm defining what is open book. Some other teacher will define open book in a different way. I'll say open book means you should only look at your textbook or look at my slides. Now, you see how it's becoming very arbitrary...They just need to copy my question and put it. They don't even need to understand my question. That's the point, and at least with the Internet, they would search, they would go through the sites. They have to look at the site and then choose some answer. Now, there's no choice also. They're learning nothing. They're not even exploring." -[T2]
% \end{quote}

% Many participants strongly feel that open-book assessment is going to lose relevance as students can easily use ChatGPT to solve them without learning anything. They suggested that the instructors should get rid of open-book assessments completely and just assess students using closed-book assessments. Some participants mentioned that they have already removed open-book assessments from their courses.

% \begin{quote}
%     Go back to paper-based tests. Make your students think. Take everything away from them. You will be saving their lives. They're going to become dumb. Go back to strict basics. Forget about all these creative components with Chat GPT around. We can't stop Chat GPT, but we'll all go back to paper-based tests because we don't want to lose this generation. - [T2]
% \end{quote}

% \noindent\textbf{Adapting open-book and open-internet assessment formats.} 
% Some participants emphasized the importance of contextualizing questions in open-internet exams and assignments to prevent ChatGPT from providing ready-made answers. Assignments that involve real observations, personal experiences, and synthesis of information may require students to demonstrate a deeper understanding and cannot be easily outsourced to AI. One participant mentioned that they try to solve the assignment using ChatGPT before releasing it to the students so as to ensure that the assignments remain challenging and promote genuine learning rather than complete reliance on AI. Another participant mentioned that instructors must also adjust the complexity of problems and assignments to make them less amenable to ChatGPT-generated solutions. Another participant mentioned that sometimes, the online information sources are inaccurate and biased which may in term trickle into the responses generated by ChatGPT. Instructors could utilize this to prepare questions or assignments that may have incorrect information widely available on the internet. This may encourage students to critically evaluate and verify information. At the same time, it may be challenging to design such assignments which are not too difficult for the weaker students. Striking the right balance between complexity and accessibility is going to be crucial.

% \begin{quote}
%     Earlier, I used to assign term papers, but now I've shifted the focus. I've added more weightage to assignments that require observation and practical involvement. Students need to write about their observations and even take real photos as part of their assignments. They can't simply rely on internet sources for everything. I emphasize these points in my assignments; for example, I ask them to include self-taken photos. This way, I can tell if they've genuinely engaged with the subject matter. I removed the term paper requirement because I know they can easily write it using ChatGPT. Secondly, in design courses, projects and assignments, most of them are not very binary; they involve observation and presentation, such as creating a video. I try to make them as non-objective as possible, so AI may not be as useful in that context. This doesn't mean I make the assignments overly challenging, but analyzing existing products or designs around them can provide valuable insights. -[T19]
% \end{quote}
 

% \noindent\textbf{Limited impact of ChatGPT on in-class closed-book assessments.} 
% Some participants were of the opinion that in-class exams are likely to remain a cornerstone of the undergraduate assessment process, with other components serving as valuable supplements. They mentioned that traditional closed-book exams as less susceptible to the influence of AI tools like ChatGPT due to the controlled and supervised nature of the testing environment. They argued that the controlled environment of in-class closed-book exam, where students are physically present and using pen and paper, ensures the integrity of the assessment process. At the same time, they also recognized that just in-class assessment is not sufficient. Other components such as assignments and projects serve to complement the assessment process and encourage students to engage deeply with course material.
% \begin{quote}
%     We usually don't rely heavily on anything for grading, especially take-home assignments. They are a component, but their purpose is to instill seriousness in the students. Maybe I'm old-fashioned, but I firmly believe that in-classroom testing is the most reliable form of assessment. Out-of-classroom testing can't be relied upon too much. So, I doubt that ChatGPT has any significant role to play because with pen and paper, when you're sitting in an exam, everything is easily manageable and under our control. -[T3]
% \end{quote}

% Continuous Monitoring and Adaptation: Instructors are actively monitoring and adapting their assignments based on ChatGPT's responses. This ongoing process helps ensure that assignments remain challenging and promote genuine learning rather than reliance on AI.

\subsubsection{\textbf{Recommendations for improving ChatGPT}}\hfill\\

\noindent\textbf{Enhancing ChatGPT for More Effective and Accountable Interactions.} Participants suggested that \textbf{ChatGPT should provide confidence scores with its responses} to help users assess the reliability of the information. Some participants also proposed that \textbf{ChatGPT should provide references or citations for the specific sources which it has used to generate a particular response}, ideally in a journal-style in-line citation format. These features would make ChatGPT more accountable as well as enable users to make informed decisions when consuming ChatGPT-generated content. Few participants also suggested that users should be encouraged to cite ChatGPT as a source in their research articles, increasing awareness about AI-generated information. Participants envisioned ChatGPT evolving to offer richer and more interactive educational experiences, including \textbf{multimedia content and spoken interactions}. They suggested integrating imagery, graphical content, animations, and spoken conversations to enhance the learning experience and provide a more dynamic and engaging user interaction compared to just text-based interactions.
Some participants recognized the challenges of inputting mathematical queries into ChatGPT and recommended improving the interface for easier input of mathematical formulas and equations. This will make ChatGPT more convenient for users seeking solutions to mathematical problems.
\begin{quote}
I think there should be some accountability...[...]...because the problem that I can see is that if ChatGPT, if it is so powerful, and in the future, if people see it as a replacement for Google, then...it can also generate biased information. Like, who will be accountable for that? So here when you do the Google search, Google itself is not providing any information; it can point to different blogs or something, and you know the identity of, know whether those people are reliable or not? Even like the media house and all, like, some media house can be biased, some can be...unbiased, so you can look at different media houses, then you can build your understanding about, like, what is what. But if instead of, if everything is a black box, and then you're just getting some information, and then that is a bit problematic, so… [T12]
\end{quote}

% \noindent\textbf{Assigning confidence score for each response.} Some participants mentioned that it would be great if ChatGPT can also provide some kind of confidence score along with its responses so that the user can consume the responses accordingly.

% \noindent\textbf{Ensuring accountability and liability.} Participants also mentioned that there should be accountability for the information generated by ChatGPT. ChatGPT should give references or cite the specific sources which it has used to generate a particular response. One participant mentioned that it would be good to have journal-style in-line citations in ChatGPT's responses where ChatGPT is able to cite the source for each sentence or a group of sentences in its response. Additionally, anyone using ChatGPT's responses should cite ChatGPT as one of their sources of information for their research articles. This would increase people's awareness about the information being generated by AI and will also help address concerns about potential misuse, fake news, and biased information. 

% \begin{quote}
% I think there should be some accountability...[...]...because the problem that I can see is that if ChatGPT, if it is so powerful, and in the future, if people see it as a replacement for Google, then...it can also generate biased information. Like, who will be accountable for that? So here when you do the Google search, Google itself is not providing any information; it can point to different blogs or something, and you know the identity of, know whether those people are reliable or not? Even like the media house and all, like, some media house can be biased, some can be...unbiased, so you can look at different media houses, then you can build your understanding about, like, what is what. But if instead of, if everything is a black box, and then you're just getting some information, and then that is a bit problematic, so… [T12]
% \end{quote}

% \noindent\textbf{Enabling Multi-Model Interactions.} Participants mentioned that ChatGPT could further evolve to offer richer and more interactive educational experiences, including multimedia content and spoken interactions. One participant mentioned that currently, ChatGPT's outputs are primarily in the form of theoretical text and suggested that it could be helpful if ChatGPT is able to integrate imagery and graphical content. They mentioned that innovative ways of presenting information, such as animations and pictorial representations, could enhance the learning experience. Another participant suggested that ChatGPT should be more interactive, allowing users to have spoken conversations with it and receive spoken responses. This would provide a more dynamic and engaging user experience compared to just text-based interactions.

% \begin{quote}
%     Let's say to present a thing, there can be different innovative ways to do that through a pictorial thing or to present it through some animation. So, if those things can be integrated into ChatGPT, that will be quite helpful because these days it is mostly text-only. More graphical things can be integrated. - [T6]
% \end{quote}

% \noindent\textbf{Improving ChatGPT for Mathematical content.} Participants also mentioned that it can be challenging to input mathematical queries effectively into ChatGPT, and they suggest improving the interface to allow for easier input of mathematical formulas and equations. This would make it more convenient for users seeking solutions to mathematical problems.

% \begin{quote}
%     If you are trying to find solutions for mathematical questions, like in Google search, we see that it's not that easy to write a mathematical formula and search for the solution. So, I think this kind of solution will also be difficult to find using ChatGPT. So maybe some improvement could be an interface which allows... -[T18]
% \end{quote}

\noindent\textbf{ChatGPT as a foundation for specialized chat-bots.} Participants noted that ChatGPT could serve as a foundation for various new tools and applications. Just as Google provided a window to the world, ChatGPT is seen as a foundational technology upon which new tools can be built. These tools could be domain-specific and tailored to the needs of researchers, students, developers, data scientists, and more. For example, \textbf{student-focused version of ChatGPT} would not simply provide answers but act as a tutor, giving hints, directions, and clarification. This approach aims to strike a balance between saving students time on redundant tasks and promoting active learning by not providing complete solutions right away. 

\begin{quote}
    Currently, there is a single ChatGPT, right? And it's based on a universal model. In the long run, probably what we will see, and this might not be good for the company as such, is a lot of chatbots tied to different objectives. There might be a chatbot that is just for helping people with assignments. There might be a chatbot that is designed for instructors to improve their questions. - [T7]
\end{quote}


\noindent \textbf{A fair and unbiased ChatGPT.} Participants expressed concerns about potential bias in the training data of ChatGPT, especially with regards to its applicability in regions that may not have been adequately represented in the data. They suggested that fairness, bias, and transparency should be thoroughly reviewed in the training process. \textbf{Addressing bias, ensuring representation from diverse sources, and providing transparency and explainability in AI systems} are crucial steps to ensure their responsible and ethical use in various contexts, including regions outside the primary training data sources.

\begin{quote}
    Working in a developing country, also called a third-world country, it is my apprehension that there may not be sufficient fairness in ChatGPT's training. They may not have used a sufficient amount of data from the region where perhaps they could not reach out to sufficiently enough. And therefore, it has been trained on, let's say, data from the US, and that may not directly apply to the real-life cases in our setting. So, I mean, my suggestion would be that fairness, you know, in their training, that should be reviewed. What data they have collected, where they have collected from, whether sufficient attention has been paid to fairness and bias, transparency, it is called explainability. I think that's kind of a standard thing which everyone is..." [T9]
\end{quote}







% ------------------------------------------------------------------------------------------------------------


